Non-intrusive and Unconstrained Keystroke Inference in VR Platforms via Infrared Side Channel

Virtual Reality (VR) technologies are increasingly employed in numerous applications across various areas. Therefore, it is essential to ensure the security of interactions between users and VR devices. In this paper, we disclose a new side-channel leakage in the constellation tracking system of mainstream VR platforms, where the infrared (IR) signals emitted from the VR controllers for controller-headset interactions can be maliciously exploited to reconstruct unconstrained input keystrokes on the virtual keyboard non-intrusively. We propose a novel keystroke inference attack named VRecKey to demonstrate the feasibility and practicality of this novel infrared side channel. Specifically, VRecKey leverages a customized 2D IR sensor array to intercept ambient IR signals emitted from VR controllers and subsequently infers (i) character-level key presses on the virtual keyboard and (ii) word-level keystrokes along with their typing trajectories. We extensively evaluate the effectiveness of VRecKey with two commercial VR devices, and the results indicate that it can achieve over 94.2% and 90.5% top-3 accuracy in inferring character-level and word-level keystrokes with varying lengths, respectively. In addition, empirical results show that VRecKey is resilient to several practical impact factors and presents effectiveness in various real-world scenarios, which provides a complementary and orthogonal attack surface for the exploration of keystroke inference attacks in VR platforms.

==> tables/comparison_prior_works.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{ccccccc}
\toprule
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}VR Keystroke\\ Inference Attacks\end{tabular}}} & \textbf{Attack Surface} & \textbf{Side Channel} & \textbf{Non-Intrusive}  & \textbf{\begin{tabular}[c]{@{}c@{}}No Fixed Position\\ of VR User\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}w/o Model\\ Inference\end{tabular}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Unconstrained\\ Inference\end{tabular}}} \\ \midrule\midrule
\multicolumn{1}{c!{\vrule width 0.5pt}}{TyPose~\cite{slocum2023going}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Motion sensors in VR headset} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Malware} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c}{\textcolor{darkred}{\xmark}} \\ %\midrule
\multicolumn{1}{c!{\vrule width 0.5pt}}{Zhang \etal~\cite{zhang2023s}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Motion sensors in VR headset} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Malware} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c}{\textcolor{darkred}{\xmark}} \\ %\midrule
\multicolumn{1}{c!{\vrule width 0.5pt}}{Wu \etal~\cite{wu2023privacy}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Motion sensors in VR headset} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Malware} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c}{\textcolor{darkred}{\xmark}} \\ %\midrule
\multicolumn{1}{c!{\vrule width 0.5pt}}{HoloLogger~\cite{luo2022holologger}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Motion sensors in VR headset} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Malware} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c}{\textcolor{darkgreen}{\cmark}} \\ %\midruleMeteriz
\multicolumn{1}{c!{\vrule width 0.5pt}}{VR-Spy~\cite{al2021vr}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Wi-Fi channel state data} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Wi-Fi CSI data} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c}{\textcolor{darkred}{\xmark}} \\ 
\multicolumn{1}{c!{\vrule width 0.5pt}}{Meteriz-Y{\i}ld{\i}ran \etal~\cite{meteriz2022keylogging}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Users' hand gestures} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Hand tracker/Camera} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c}{\textcolor{darkred}{\xmark}} \\
\multicolumn{1}{c!{\vrule width 0.5pt}}{Su \etal~\cite{su2024remote}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Unencrypted Photon protocol} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Network traffic} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c}{\textcolor{darkgreen}{\cmark}} \\
% \multicolumn{1}{l!{\vrule width 0.5pt}}{VR-Spy~\cite{al2021vr}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Wi-Fi channel state data} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Wi-Fi CSI data} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c}{\textcolor{darkred}{\xmark}} \\ 
%\midrule
\multicolumn{1}{c!{\vrule width 0.5pt}}{Gopal \etal~\cite{gopal2023hidden}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Video of VR users' gestures} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Camera} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c}{\textcolor{darkred}{\xmark}} \\ 
%\midrule
\multicolumn{1}{c!{\vrule width 0.5pt}}{Heimdall~\cite{luo2024eavesdropping}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Sound from VR controllers} & \multicolumn{1}{c!{\vrule width 0.5pt}}{Acoustic signal} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkred}{\xmark}} & \multicolumn{1}{c}{\textcolor{darkred}{\xmark}} \\ %\midrule
\midrule
\multicolumn{1}{c!{\vrule width 0.5pt}}{\textbf{\sysname}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{IR signals from VR controllers} & \multicolumn{1}{c!{\vrule width 0.5pt}}{IR signal} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c!{\vrule width 0.5pt}}{\textcolor{darkgreen}{\cmark}} & \multicolumn{1}{c}{\textcolor{darkgreen}{\cmark}} \\ \bottomrule
\end{tabular}%
\vspace{-0.05in}
\caption{Comparison with related keystroke inference attacks in VR devices. ``\textcolor{darkgreen}{\cmark}'': Yes, ``\textcolor{darkred}{\xmark}'': No.}
\vspace{-0.35in}
\label{tab:comparison_prior_works_v3}
\end{table*}
